Bit Distribution Study and Implementation of Spatial Quality Map in the JPEG-AI Standardization

Currently, there is a high demand for neural network-based image compression codecs. These codecs employ non-linear transforms to create compact bit representations and facilitate faster coding speeds on devices compared to the hand-crafted transforms used in classical frameworks. The scientific and industrial communities are highly interested in these properties, leading to the standardization effort of JPEG-AI. The JPEG-AI verification model has been released and is currently under development for standardization. Utilizing neural networks, it can outperform the classic codec VVC intra by over 10% BD-rate operating at base operation point. Researchers attribute this success to the flexible bit distribution in the spatial domain, in contrast to VVC intra's anchor that is generated with a constant quality point. However, our study reveals that VVC intra displays a more adaptable bit distribution structure through the implementation of various block sizes. As a result of our observations, we have proposed a spatial bit allocation method to optimize the JPEG-AI verification model's bit distribution and enhance the visual quality. Furthermore, by applying the VVC bit distribution strategy, the objective performance of JPEG-AI verification mode can be further improved, resulting in a maximum gain of 0.45 dB in PSNR-Y.

==> sections/VM.tex <==
\section{JPEG-AI verification Model}
The first version of JPEG AI verification model (JPEG AI VM1.0) is described in \cite{VM1.0}. JPEG AI VM1.0 has been approved in the $97^{th}$ JPEG meeting and it is the 3rd version of the JPEG AI Verification model under Consideration (VMuC). VMuC contains as many tools as possible from the two best-performing JPEG AI CfP responses \cite{jpegaiteam14} \cite{JpegaiBDCFP}. In this section, the main structure of JPEG AI VM1.0 tool-off configuration will be introduced, and on top of VM1.0, the changes from VM2.0 will be shown.

\begin{figure}[t]
	\centerline{\includegraphics[trim=1.089cm 4.248cm 1.198cm 0cm, clip,width=1.0\linewidth]{images/model.pdf}}
	\caption{Example structure of CCS \cite{jia2022learningbased}. ``AE'' and ``AD'' indicate arithmetic encoder and arithmetic decoder. ``Q'' denotes the quantizer, ``DS'' stands for down-sampling. ``cat'' is used for channel-wise concatenation. Here, the codec for the Y component uses 128 channels and the one for the UV component uses 64 channels. For simplicity, the hyperprior and the context model are omitted. }
	\label{figfullcodec}
\end{figure}

\subsection{Conditional Color Separation Frame Work} \label{CCS}
The concept of Conditional Color Separation (CCS) has been published by Jia et al.\cite{jia2022learningbased} and will be used as the base framework. In this base framework, the different color components are separated into primary and secondary groups. Primary and secondary color components are processed separately by using the same network architecture, and the codec for the primary color components has more channels of the latent tensor. When processing the secondary color components, the information from the primary color components is used as the auxiliary information. 

In VM1.0, the input image will be firstly converted from RGB to YUV420 format according to BT.709, thus, the internal color format is YUV420. Because in YUV420, the luminance (Y) component has a bigger size than chroma (UV) components, luminance is assigned to the primary color component and chroma is the secondary color component. To maintain the information from luminance, more channels are assigned for Y than for UV. Number of channels of latent tensor is $C_y = 128$, and for UV is $C_{uv} = 64$, and UV are jointly coded. When UV uses Y information as the auxiliary input, Y needs to be downsampled because of its bigger size. The basic illustration is shown in Fig. \ref{figfullcodec}


\subsection{Decoupled Parsing and Reconstruction Scheme } \label{codec one color}
\begin{figure*}[t]
	\centerline{\includegraphics[width=1.0\linewidth]{images/JPEG_AI_model.png}}
	\caption{JPEG AI learning-based codec (without tools)\cite{VM1.0}. Dash arrows and boxes correspond to encoder operations. }
	\label{figJPEGAI}
\end{figure*}
Fig. \ref{figJPEGAI} shows the decoupled scheme of the primary color component in VM1.0. Different from the other NN-based image codecs, this scheme doesn't request an autoregressive entropy model, the entropy coding parameters can be independently generated from the latent tensor decoding.

The input image will be first processed by an analysis transform net, after that the latent tensor $y$ is obtained. Then $y$ will be the input of the hyper encoder net and the hyper latent tensor $z$ will be generated. The first pair of arithmetic codecs can generate bitstream #1 from $z$ and reconstruct $\hat{z}$ on the decoder side. Hyper decoder net takes $\hat{z}$ as input and provides the input of the prediction fusion net. Besides, prediction fusion net takes the output from context model net as well and generates the prediction $\mu$ of $y$. The difference between $y$ and $\mu$ is the residual $r$, after quantization of $r$, $\hat{z}$ will be transferred to bitstream #2 by the arithmetic codec. To help the entropy model predict the distribution of the signal, the hyper scale decoder Net takes $\hat{z}$ and output variance $\sigma$ of the entropy model.

For the secondary color components, the codec architecture is similar to the primary color components. Besides, it requests the auxiliary information from the primary color component before analysis transform net and the latent presentation of the auxiliary information before synthesis transform net.

\subsection{Variable Rates Capability}
To cover a long bit range, four checkpoints are trained for VM1.0. Four checkpoints are trained with four different $\beta$s. $\beta$ is the trade-off parameter in the loss function: $L = R + \beta \cdot D $, where $R$ is the rate and $D$ is the distortion between the original and reconstructed image. 

A gain unit is applied on VM1.0 for the precise bit rate matching. It is proposed by Cui et al. \cite{cui2020g}. And in VM1.0 the extrapolation gain unit is implemented. In Fig. \ref{figJPEGAI} two pairs of forward and inverse gain vectors $\{ m_t, {m_t}^{-1}\}$ are built in the primary and secondary color components codec. Each gain unit $m_t$ has multiple gain vectors $m$, and $m$ is a channel-wise quantization map with the same number of channels in the latent space, thus all elements in one channel use the same quantization scaling factor. 

During the training, one gain vector is updated with one specific beta, and multiple betas ($\beta \in \{\beta_t\}$) will be trained in the variable training stage. Thus, for each checkpoint, at least one gain vector in the gain unit will be updated.

During the inference, to match the target bit rate point, a new $\beta_v$ will be calculated by the Bit Rate Matcher. If $\beta_v \notin \{\beta_t\} $, a new gain vector $m_v$ will be calculated by the existing $m_t$. If the $\beta_v$ is bigger than $\beta_{min}$ or smaller than $\beta_{max}$ in $\{\beta_t\}$, then $m_v$ is calculated by extrapolation way as $m_v = m_t \times \frac{\beta_v}{\beta_t}$. If the $\beta_v$ is in the range of $\{\beta_t\}$, it can be found by the nearest reference $\beta_l < \beta_v < \beta_h$, and calculated by $m_v = m_t \times \frac{\beta_v - \beta_l}{\beta_h - \beta_l}$.

\subsection{Difference between JPEG-AI VM1.0 and VM2.0}
JPEG-AI VM2.0 has an update on JPEG-AI VM1.0 from the standardization group, some updates are for the tool-on configuration, and some are for the tool-off configuration. Since our experiments are focused on the tool-off configuration, here two main changes for tool-off configuration will be introduced.

The first change is from Solovyev et al. \cite{wg1m98040} and Yang et al. \cite{wg1m98092}, where an additional gain unit after the hyper scale decoder is added. Thus, $\sigma$ of the entropy model has the distribution in the same scale as the latent tensor $y$.

The second main change is from Alshina et al. \cite{wg1m98019}, it changed the channel number in Prediction Fusion Net and Hyper Scale Decoder Net and aligned to the power of 2. It enhances the stability of the codec.

In the rest part of the paper, we will use JPEG-AI VM to represent JPEG-AI  VM2.0.




teamp for figure

% \subfloat[reconstructed image of JPEG-AI VM \protect \\ PSNR-Y 41.45 dB   \label{fig:img05_a}]{\includegraphics{images/VM_00005_TE_1336x872_8bit_sRGB_075.png} }\hfil
% \subfloat[original image     \label{fig:img05_b}]{\includegraphics{images/00005_TE_1336x872_8bit_sRGB.png} }\hfil
% \subfloat[reconstructed image of VVC PSNR-Y 46.73 dB  \label{fig:img05_c}]{\includegraphics{images/VVC_00005_TE_1336x872_8bit_sRGB_8bit_sRGB_075.png} }\hfil

% \caption{Original and reconstructed image 00005 at 0.75 bpp}
% \label{fig:img05}

\begin{figure*}
    \centering
    \setkeys{Gin}{width=0.3\linewidth} % <---

\subfloat[BDM of JPEG-AI VM \label{fig:BDM_12_a}]{\includegraphics{images/img32_75_VM_BDM.jpg} }\hfil
\subfloat[original BDM of VVC \label{fig:BDM_12_b}]{\includegraphics{images/img32_75_VVC_BDM.jpg} }\hfil
\subfloat[regrouped $16\times 16$ block BDM of VVC \label{fig:BDM_12_c}]{\includegraphics{images/img32_75_VVC_BDM_16.jpg} }

\caption{Luminance BDM of image 32 at 0.75 bpp}
\label{fig:BDM_12}
\end{figure*}


%% temp of complex quality map
\subsection{Complex Quality Index Map Result}
The previous section \ref{ROI_sec} demonstrated the utilization of a spatial quality index map for ROI-based coding. This technique utilizes only two distinct levels of quality in the index map, however, for other scenarios employing a more intricate quality index map, the cost of bits may be of interest to individuals. 

To examine the bit cost of a more intricate quality index map, we generated a quality index map with 5 different index levels and a complex texture. The chart, depicted in Fig. \ref{compQP}, displays a quality index with a quantization index ranging from -4 to 0, with darker areas indicating a lower quantization index. The quality index chart is generated by determining the variance of luminance in each $16\times16$ block and subsequently quantized into five levels. The codec uses a total of 0.843 bpp to process the test image. In addition, 0.011 bpp of the total are allocated for transmitting the quality index map. Therefore, the quality map accounts for 1.31\% of the total bits used. 

From this experiment, we observed that implementing a more advanced quality index map did not significantly increase the bit cost.

\begin{figure*}[t]
	\centerline{\includegraphics[width=0.95\linewidth]{images/complex_QP.pdf}}
	\caption{Bits cost of the test image and its quality index map}
	\label{compQP}
\end{figure*}

